Federated Foundation Models on Heterogeneous Time Series

Training a general-purpose time series foundation models with robust generalization capabilities across diverse applications from scratch is still an open challenge. Efforts are primarily focused on fusing cross-domain time series datasets to extract shared subsequences as tokens for training models on Transformer architecture. However, due to significant statistical heterogeneity across domains, this cross-domain fusing approach doesn't work effectively as the same as fusing texts and images. To tackle this challenge, this paper proposes a novel federated learning approach to address the heterogeneity in time series foundation models training, namely FFTS. Specifically, each data-holding organization is treated as an independent client in a collaborative learning framework with federated settings, and then many client-specific local models will be trained to preserve the unique characteristics per dataset. Moreover, a new regularization mechanism will be applied to both client-side and server-side, thus to align the shared knowledge across heterogeneous datasets from different domains. Extensive experiments on benchmark datasets demonstrate the effectiveness of the proposed federated learning approach. The newly learned time series foundation models achieve superior generalization capabilities on cross-domain time series analysis tasks, including forecasting, imputation, and anomaly detection.

==> Table/anomaly_detection_federated.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[tbh]
  \centering
    \begin{tabular}{ccccccr}
    \toprule
    Method & SMD   & MSL   & SMAP  & SWaT  & PSM   & \multicolumn{1}{c}{Avg F1} \\
    \midrule
    FedAvg &       &       &       &       &       &  \\
    FedProx &       &       &       &       &       &  \\
    pFedMe &       &       &       &       &       &  \\
    FedTSF (Ours) &       &       &       &       &       &  \\
    \bottomrule
    \end{tabular}%
  \label{tab:addlabel}%
    \caption{Add caption}
\end{table}%

